Minimum Degree Threshold for $H$-factors with High Discrepancy

Given a graph $H$, a perfect $H$-factor in a graph $G$ is a collection of vertex-disjoint copies of $H$ spanning $G$. K\"uhn and Osthus showed that the minimum degree threshold for a graph $G$ to contain a perfect $H$-factor is either given by $1-1/\chi(H)$ or by $1-1/\chi_{cr}(H)$ depending on certain natural divisibility considerations. Given a graph $G$ of order $n$, a $2$-edge-coloring of $G$ and a subgraph $G'$ of $G$, we say that $G'$ has high discrepancy if it contains significantly (linear in $n$) more edges of one color than the other. Balogh, Csaba, Pluh\'ar and Treglown asked for the minimum degree threshold guaranteeing that every 2-edge-coloring of $G$ has an $H$-factor with high discrepancy and they settled the case where $H$ is a clique. Here we completely resolve this question by determining the minimum degree threshold for high discrepancy of $H$-factors for every graph $H$.

==> high_degree.tex <==
\begin{lemma}\label{high_degree}
$$\delta^*(H)\leq\max\{3/4,1-1/(r+1)\}$$
\end{lemma}
\begin{proof}
Let $\eta>0$ and note that we can assume that $\eta\ll 1/r$. Let $1/n_0\ll \gamma\ll\varepsilon,1/\ell_0\ll d\ll\nu\ll\gamma'\ll\eta\ll 1/r$ be positive constants defined with the described relations, where $\gamma'$ is obtained by applying Theorem~\ref{kr_discrepancy} with $H,\eta$. Let $G$ be an arbitrary graph of order $n\geq n_0$ with $n$ divisible by $|H|$ and 
$$
\delta(G)\geq(\max\{3/4,1-1/(r+1)\}+\eta)n.
$$
Let $M\subseteq V(G)$ with $|M|\leq\nu n$ be an $H$-absorbing set for any $W\subseteq V(G)\backslash M$ with $|W|\leq\nu^3$ and $|W|$ divisible by $|H|$ and let $G_0 = G[V(G)\backslash M]$. Note that such a set exists by Lemma~\ref{absorption}. Let $f$ be an arbitrary $2$-edge-coloring of $G$ and we apply Lemma~\ref{regularity} with parameters $\varepsilon,\ell_0,d$ to $G_0$ and $f$. Let $G_0'$ be the pure graph and $R_0$ the reduced graph with respect to $G_0$ and $f_{R_0}$ the corresponding $2$-edge-coloring.
Let us remove $k<r$ clusters from $R_0$ such that $|R_0|$ becomes divisible by $r$. Note that by Lemma~\ref{R_degree} and since $\varepsilon,1/\ell_0\ll d\ll\nu\ll\eta\ll1/r$, we get that
$$\delta(R_0)\geq (\max\{3/4,1-1/(r+1)\}+\eta/2)|R_0|.$$ 
By Theorem~\ref{kr_discrepancy}, there exists a perfect $K_r$-factor $F_{R_0}$ of $R_0$ with $|f_{R_0}(F_{R_0})|\geq\gamma'|R_0|$. Let $K\subseteq F_{R_0}$ be a copy of $K_r$ and let $W_1,W_2,\dots,W_r$ be the clusters of $K$ and let $m=|W_1|$. 

Then, we can delete less than $\varepsilon^{1/2}m$ vertices from each of these to obtain clusters $W_1',W_2',\dots,W_r'$ with $|W_1'|=|W_2'|=\dots=|W_r'|$ and $|W_1'|$ divisible by $(r-1)!|H|$ such that for each pair of clusters $U,V$ we have that $G_0'[U,V]^{f_R(UV)}$ is $(2\varepsilon,d/2)$-superregular.\MC{ Does this need explanation? It is not explained in \cite{balogh2021discrepancy} so I thought it might be a well-known fact but it is not 'trivial'.} Let $B_K$ be the graph on vertices $\bigcup_{1\leq i\leq r}W_i'$ with edges $\bigcup_{1\leq i<j\leq r}G'[W_i',W_j']^{f_R(W_iW_j)}$. Let $B$ be an $(r-1)!|H|$-blowup of $K_r$.
By Lemma~\ref{blowup_lemma} and for $\varepsilon>0$ small enough, there exists a perfect $B$-factor $F_1$ of $B_K$. 
Let $A_1,A_2,\dots,A_r$ be the parts of an $r$-vertex-coloring of $H$ and let $B_1,B_2,\dots,B_r$ be the clusters of $B$. Then, there exists a perfect $H$-factor $F_B$ of $B$ that contains for every permutation $\sigma:[r]\rightarrow[r]$ a copy of $H$ with the vertices of $A_i$ in cluster $B_{\sigma(i)}$ for every $1\leq i\leq r$. Note that for every $1\leq i,j\leq r$, by the symmetry of $F_B$ we have that
$$e_{F_B}(B_i,B_j) = \frac{e(H)|B|}{\binom{r}{2}|H|}.$$
Taking the $H$-factor $F_B$ of every copy of $B$ in $F_1$ gives us a perfect $H$-factor $F_K$ of $B_K$ with for every $1\leq i,j\leq r$,
$$
e_{F_K}(W_i',W_j') = \frac{e(H)|B_K|}{\binom{r}{2}|H|}.
$$
Then,
$$
f(F_K) = \frac{e(H)|B_K|}{\binom{r}{2}|H|}f_{R_0}(K)\geq\frac{e(H)n}{2\binom{r}{2}|H||R_0|}f_{R_0}(K),
$$
Where we used $|B_K|\geq n/(2|R_0|)$.
Let $F'$ be the $H$-factor in $G$ containing for every copy $K$ of $K_r$ in $F_{R_0}$ such an $H$-factor $F_K$ and let $W\subseteq V(G_0)$ be the set of vertices not contained in $F'$. Note that $|W|\leq (\varepsilon + r\varepsilon^{1/2})n\ll \nu n$. By the definition of $M$, there exists a perfect $H$-factor $F''$ in $G[M\cup W]$. Therefore, $F=F'\cup F''$ is a perfect $H$-factor in  $G$ with
\begin{align*}
|f(F)| &\geq |f(F')|-|f(F'')|\\
&\geq \frac{e(H)}{2\binom{r}{2}|H|}\cdot\frac{|f_{R_0}(F_{R_0})|}{|R_0|}n-\frac{2\nu e(H)}{|H|}n\\
&\geq \frac{\gamma'e(H)}{2\binom{r}{2}|H|}n-\frac{2\nu e(H)}{|H|}n
\geq \gamma n,
\end{align*}
where we used $\gamma\ll\nu\ll\gamma'$.
\end{proof}
